Hidden Ciphers and Where to Find Them: Static Discovery and Assessment of Cryptographic Assets in Software

Modern software systems rely on cryptography for data protection, authentication, and trust establishment, yet organizations often lack a structured view of the cryptography deployed across source code, configuration, dependencies, and cryptographic files. This lack of visibility complicates security governance and post-quantum migration planning. This paper presents a static approach for discovering and assessing cryptographic assets in software systems. We introduce a classification of Crypto-Material, Crypto-Artifacts, and Crypto-Invocations, derive an extensible scanner-independent rule repository from it, and implement a static scanner that applies these rules to produce CBOM-oriented output. We evaluate the approach on a synthetic benchmark with known ground truth and on a real-world infrastructure of ten deployed services. The scanner achieves an F1 score of 0.75 for asset discovery and correctly annotates 91% of expected weaknesses and vulnerabilities. In the realworld setting, it processes 57 610 files in under six minutes and discovers 370 cryptographic assets, including six CVE-linked vulnerabilities and 52 post-quantum migration candidates. Real-world coverage is assessed against a manually compiled reference list rather than an exhaustive one. These results show that classification-driven static discovery can provide practical cryptographic transparency for governance and post-quantum migration planning.

==> sections/02_related_work.bk.tex <==
% ============================================================
% Section 2 — Related Work
% ============================================================
\section{Related Work}
\label{sec:related_work}

We structure related work along three dimensions that correspond to the core concerns of our approach: the static detection of cryptographic usage in software, the classification and inventorying of cryptographic assets, and the assessment of discovered assets against established weakness and vulnerability taxonomies.

\paragraph{Static Detection of Cryptographic Usage.}

Static analysis is the dominant approach for detecting cryptographic usage in software because it operates without a runtime environment and scales to large codebases.
Arzt~et~al.~\cite{Arzt2015Towards} established the conceptual framing that motivates specification-driven detection: integrating cryptography correctly in software is a software engineering challenge requiring formal usage constraints, not merely a list of forbidden API names.
Building on this foundation, CrySL~\cite{Krueger2021CrySL} introduced an extensible specification language that encodes correct cryptographic API usage as machine-checkable rules over method-call sequences, predicates, and value constraints.
CryptoGuard~\cite{Rahaman2019CryptoGuard} improved detection precision through backward program slicing, achieving deployment-scale analysis of 22 classes of cryptographic misuse in large Java projects.
CRYScanner~\cite{Choudhari2022CRYScanner} further demonstrated that cryptographic misuse is often semantic and relational rather than reducible to a single forbidden API call, pushing detection toward behavior-centered analysis.
More recently, language-specific approaches have extended misuse detection to Python~\cite{Frantz2024Cryptolation,Cho2025Cryptbara}, addressing the additional challenges that dynamic language features pose for static reasoning.

A common characteristic of these approaches is that their detection scope is \emph{driven by known misuse patterns}: what is searched for is determined by what is known to be wrong.
In contrast, our goal is broad \emph{inventory generation} rather than misuse detection.
We aim to discover all cryptographic assets present in a software system, regardless of whether they relate to a known weakness, and to produce structured output suitable for governance and post-quantum migration planning.

Lightweight tools such as Wind River's Crypto Detector~\cite{windriver2020cryptodetector} and a CBOM-generation tool for the Node.js ecosystem~\cite{leirimaa2024supportingPQC} pursue a related inventory goal using keyword search and regular expression matching.
These approaches confirm the practical need for automated cryptographic discovery but provide limited structural coverage and no systematic classification of asset types.
CBOMkit~\cite{ibm2025cbomkit} operationalizes the CycloneDX~v1.7 CBOM schema for Java, Python, and Go source code and container images, supporting CBOM generation, compliance checking, and visualization.
However, its detection scope is limited to source-level invocations and does not extend to structured cryptographic artifacts such as certificates and keystores, or to opaque cryptographic material such as private keys and seeds.

Beyond source code, several approaches target cryptographic usage in compiled binaries and firmware: Where's Crypto?~\cite{meijer2021whereIsCrypto} uses data-flow graph isomorphism, CrypTody~\cite{Wang2024CrypTody} extends misuse analysis to IoT firmware, and Rattanavipanon~et~al.~\cite{rattanavipanon2025toolchainPQC} propose a PQC migration toolchain for binary-level analysis.
These approaches operate on a fundamentally different artifact type; our work focuses on software systems at rest — source code, configuration, dependency metadata, and cryptographic file formats.

Dynamic analysis offers complementary coverage by observing actual runtime values.
CRYLOGGER~\cite{Piccolboni2020CryLogger} instruments Android applications at runtime to log cryptographic API parameters and validate them offline against crypto rules, capturing concrete parameter values that static analysis cannot resolve.
While dynamic analysis can reveal actual usage rather than potential usage, it requires a running environment and cannot be applied to offline repositories or systems at rest.
Our approach is deliberately static, trading runtime completeness for determinism, offline applicability, and integration into CI/CD pipelines.

Our approach differs from all of the above by targeting three structurally distinct asset categories in a single static pipeline and by externalizing all detection and assessment logic into a dedicated, scanner-independent repository.
No existing approach combines these three aspects: a systematic asset classification, a decoupled rule repository, and CBOM-oriented output across material, artifact, and invocation types.

\paragraph{Classification and Inventorying of Cryptographic Assets.}

Producing a meaningful cryptographic inventory requires a clear answer to a prior question: \emph{what} constitutes a cryptographic asset in software and how should it be classified for discovery?
Existing work largely leaves this question implicit.
The CycloneDX~v1.7 CBOM schema defines how cryptographic assets are \emph{represented} in a bill of materials, but does not prescribe a classification that drives \emph{how} they should be found.
Schmitt~et~al.~\cite{schmitt2024CriteriaToolingCryptoInventories} identify criteria and tooling requirements for generating cryptographic inventories and propose a prototype covering package managers and hardware-level detection, but do not derive a systematic, discovery-oriented asset taxonomy as a foundation for detection rules.

Without an explicit classification, it is difficult to determine what coverage a scanner achieves, what asset types remain undiscovered, and how findings from different tools can be compared.
Our work addresses this gap by establishing a classification that distinguishes three structurally distinct categories — Crypto-Material, Crypto-Artifacts, and Crypto-Invocations — and derives detection and assessment rules directly from it.

\paragraph{Weakness and Vulnerability Taxonomies for Cryptographic Assessment.}

Assessing discovered cryptographic assets against known security issues requires grounding in established taxonomies.
The MITRE CWE taxonomy provides a structured vocabulary for cryptographic weaknesses, including CWE-327 (use of a broken or risky cryptographic algorithm), CWE-321 (use of hard-coded cryptographic keys), and CWE-338 (use of a cryptographically weak pseudo-random number generator).
OWASP A02:2021 Cryptographic Failures provides a complementary, application-oriented view.
Existing scanners typically treat these taxonomies as their \emph{primary detection scope}: a finding is only reported if it maps to a known weakness class.
Empirical evaluations have shown that even state-of-the-art misuse detectors leave important finding classes uncovered~\cite{Afrose2019CryptoAPIBench,Zhang2023AreWeThereYet}, which limits the completeness of any inventory derived solely from weakness-driven detection.

Our approach inverts this relationship.
We first discover and inventory cryptographic assets across all three categories, regardless of whether they relate to a known weakness or vulnerability.
Assessment — the mapping of discovered assets to CWE entries, CVE records, and severity ratings — is applied as a \emph{subsequent and independent step} in the pipeline.
This separation ensures that the discovery scope is not artificially constrained by the current state of weakness taxonomies, and that the resulting inventory remains useful even where no known weakness applies.

